A Secure Cloud with Minimal Provider Trust

Bolted is a new architecture for a bare metal cloud with the goal of providing security-sensitive customers of a cloud the same level of security and control that they can obtain in their own private data centers. It allows tenants to elastically allocate secure resources within a cloud while being protected from other previous, current, and future tenants of the cloud. The provisioning of a new server to a tenant isolates a bare metal server, only allowing it to communicate with other tenant's servers once its critical firmware and software have been attested to the tenant. Tenants, rather than the provider, control the tradeoffs between security, price, and performance. A prototype demonstrates scalable end-to-end security with small overhead compared to a less secure alternative.

==> docs/archold.tex <==
\section{Design Requirements and Architecture}\label{arch_sec}
\label{docs:arch}

Our goal is to create a secure enclave on bare metal in a cloud that disrupts attacks against confidentiality, integrity, and availability (CIA). We want do this while trusting the cloud provider as little as possible.

To get this done, three major conditions should be satisfied: \textbf{Node integrity} to prevent a previous tenant from leaving something in the machine that can disrupt tenant's enclaves CIA. \textbf{Network protection} to protect against a network attacker. And \textbf{Storage protection} to ensure that an attacker (e.g., next tenant) can't read anything the current tenant leaves behind.

Now, we can talk about how to accomplish the 3 core conditions for a secure enclave. At a high level, the tenant asks the node allocator for a machine. The node allocator gives the tenant a node that is in the "airlock state". Before adding this node to the tenant's network, it needs to attest node's firmware integrity. Airlock state means that tenant has not admitted the node into its secure enclave yet. Once the tenant attests the node, it admits the node into its secure enclave and starts trusting it. At this time, the tenant needs to take this not quite booted up attested node and put its OS/data on it with the provisioning service. If the node failes the attestation, it will be rejected and put in the rejected list. Once the node is in the secure enclave, the tenant can continue to attest its state and oust the node from its enclave and revoke it's access to data and network if anything goes wrong. 


%Previous works have shown that we can do a minimal bare metal cloud with just a node allocator and network configurator. \textcolor{red}{Should it be here?} For example, HIL To make this usable and fast, we also need to have a flexible and nimble provisioning service (e.g., BMI).

%We've designed this general bare metal enclave concept to allow different implementations of these components to be used depending on security, performance, trust etc...

%Bolted consists of four main components. After describing these components, this section explains the transitions between the states nodes can be in. We then discuss how the components can be deployed in different ways to support different security requirements. The second half of this section describes the role of the four components.


\subsection{Components}
The architecture of Bolted, shown in Figure \ref{fig:simple}, is composed of three main components. \textcolor{red}{The figure should be updated.}

\begin{itemize}
	\item \textbf{Isolation Service} allocates nodes to tenants. It also configures networks to isolate the nodes allocated to different tenants. 
	\item \textbf{Attestation Service} measures the code running on a node, produces a hash of the code, and checks that hash against a whitelist. 
	\item \textbf{Provisioning Service} is used to install tenant software on the node, from bootloaders to operating systems.
	%\item \textbf{Orchestration Engine} automates the sequence of operations needed to provision a secure node. These operations involve the above mentioned services, however, the tenant can and does directly call the underlying services when needed. 
\end{itemize} 

\subsection{States of a node}
In Bolted's architecture, a node transitions between the following states.

\begin{itemize}
	\item \textbf{Free:} A node not allocated to any tenant.
	\item \textbf{Airlock:} In this state a node is quarantined i.e. not connected to the requesting tenant networks. The airlock state is used to ensure that the node's firmware is not compromised before connecting the node to tenant networks.
	\item \textbf{Allocated:} This refers to a state when the node is connected to tenant networks.
	\item \textbf{Rejected:} Any node which fails firmware attestation is rejected. All infected nodes are rejected and isolated from the rest of the cloud for cleaning purposes. Any cleaning activity will take place here before a node can be transition to the Free state.
\end{itemize}

\subsection{Isolation Service}
The Isolation Service allocates nodes and networks, and communicates with the network switches to connect nodes to those networks using isolation techniques e.g., VLANs or VXLANs. The Isolation Service ensures that the nodes in the Free state are not part of any network. The Isolation Service creates a new separate network when the node is put in the Airlock state, and puts the node, the Attestation Service and the Provisioning Service on this network. Finally, when the node is in Allocated state, the Isolation Service disconnects it from the temporary Airlock network and makes it part of the tenant networks.

The Isolation Service uses network isolation instead of encryption based logical isolation in order to enforce guarantees of performance and protect against traffic analysis attacks. Since all these operations have to be carried out in switches and thus are privileged, they can only be done by the cloud provider. 

\subsection{Attestation Service} 
To ensure that a node has trusted firmware, the firmware can be either \textbf{verified} or \textbf{attested}; Bolted uses the attestation method. This takes place in the Airlock state and employs the TPM technology which places the root of trust in the hardware.
%With verification, software is signed by its vendor's key and that signature can be verified but the tenant has no insight into the process. Verification has to be done by embedded programs which cant often communicate with online authorities and there is always the threat of infected components being signed by an attacker with the vendor's key. 
With attestation, every piece of software is hashed and the value is checked against a precomputed whitelist. Any altered code will result in a different hash and thus not pass the attestation. 
%This allows for any kind of code to be measured, the values can be recorded for auditing purposes and offers more flexibility to the tenant. 
%While verification can be a good complement to attestation, it is not sufficient in and of itself. As we will see, we have succeeded in bypassing verification in our own systems, and a malicious provider can easily do the same. 
%Bolted provides security through \textit{attestation}: measuring firmware and software on a node and comparing it against a whitelist to ensure that the code is unchanged. 

%When the node is in Airlock state, it is on the same network as the Attestation and the Provisioning Services. Here, in the initial stages of boot sequence, client side of the attestation software is provisioned into the node. This client measures the firmware, itself and any other code present such as the boot loader etc. These measurements are saved into the Platform Configuration Registers (PCRs) \cite{needed} through the TPM. These stored values are then sent to the Attestation Service in the form of a TPM quote \cite{needed}, which then matches them to a whitelist. Infected firmware or other code will not match with the whitelist and so the infected node will be rejected.

The root of trust for attestation service lies in the hardware by making use of the TPM which is a tamper resistant piece of hardware. When the measurement values are sent to the Attestation Service as a TPM quote, this quote is signed with a unique key by the TPM. This signature can't be forged \cite{needed} and thus the root of trust lies in the secure hardware. In Bolted's architecture, the Attestation Service can be deployed by the tenant decreasing the need to trust the provider.

Once the hardware root of trust is established, the tenant builds a chain of trust; every step in the boot sequence will be attested including the operating system and applications. Further, the tenant can periocially check if the entire software stack running on the node is unaffected. This is done through \textbf{Continous Attestation} where the attestation client periodically measures the code running on the node and stores the values in the PCRs. These values are sent to the Attestation Service as TPM quote which checks them against a whitelist. %This is fundamentally more challenging in a provider deployed attestation service where the tenants would need to upload the white list for their operatings systems and software to the provider Attestation Service; hence we really only assume continous attestation for the untrusting tenants who have their own deployment of the Attestation Service.

\subsection{Provisioning Service}
The Provisioning Service is used to set up the nodes by installing software on them. The Provisioning Service works in two steps; initial provisioning and then further provisioning. Initial Provisioning takes place in the Airlock state, where the bootloader and client side attestation software are provisioned into the node. This is necessary in order to carry out firmware attestation and thus central to Bolted's architecture. Once the firmware is attested, the node is moved out of the Airlock and made part of the tenant networks. Here further provisioning occurs and tenant's operating system and any other required software are installed on the nodes. The node becomes ready to use for the tenant. %The Provisioning Service can also be deployed by the tenant.


%\subsection{Orchestration Engine}
%Orchestration Engine automates all the different steps for allocation, attestation and provisioning of a secure node. Orchestration Engine does not abstract the functionality of any underlying service, instead it only provides an automated way to get a secure node. The tenant can and will still directly invoke the other services if need arises, as discussed later. Orchestration Engine can be deployed by the tenant. 

\textcolor{red}{Amin: we need to talk about storage encryption here.}


==> docs/background.tex <==
\section{Background}\label{doc:background}
It is relatively straightforward to imagine setting up security frameworks in a virtualized environment because there is a fully deployed guest OS environment to work in. Even at a hypervisor level, there is a host OS beneath it to provide a working environment. Bare metal clouds on the contrary do not have the luxury of a working environment. By definition, tenants get bare metal nodes and any pre-existing security software on those nodes goes against the design goals we set up for ourselves. It would lead to increased trusted computing base, persistent code which could be compromised and finally placing more trust in the cloud provider for correct deployment of this software.

So, in order to work with actual bare metal nodes, we need a mechanism to allocate nodes and configure network. We also need a mechanism to quickly provision non persistent, fresh security software to examine the node for any threat. This service can be tenant owned to avoid any trust in the provider. Finally we need an attestation service which can ensure that the firmware in the node or any other software is not compromised. We use existing solutions to this end which are described below.

\subsection{Hardware Isolation Layer}
Hardware Isolation Layer or HIL \cite{hil} is a thin, exo-kernel like layer for the cloud designed to provide allocation of resources and their isolation from each other without manual administrative effort. HIL is not a provisioning service, rather any provisioning service (e.g., M2, Ironic, xCAT and etc.) can work on top of HIL and directly interact with the underlying hardware.

\subsection{Bare Metal Imaging}
Bare Metal Imaging or BMI \cite{bmi} is a lightweight and fast provisioning service that uses network boot to provision tens of nodes under two minutes, and can decommission and re-purpose unused/underutilized nodes under 10 minutes.

\subsection{Keylime}
Keylime \cite{keylime} is a cloud key management and ditribution system for secure provisioning and monitoring. It leverages TPM and vTPM technology to validate the integrity of software running on a cloud node. \newline 

\noindent It must be noted that other services can be use instead of the three listed above. The main idea is to provide a bare minimum working environment so that the security guarantees can be provided.


==> docs/goals.tex <==
\section{Design Goals}
\label{docs:goals}

Users have important data and code residing in public clouds. Security conscious users want to trust as few entities as possible but other users who are not as concerned about security might just want a flawless experience using the cloud. A cloud provider therefore has to trade-off security with usability in order to maximize both types of users. Therefore, it is necessary to discuss design goals which need to met before building such a cloud which provides security as a service to interested users.

\begin{enumerate}
	\item \textbf{Service} \label{goal: service} As mentioned earlier, users should have the option of choosing security. It should not be mandatory for everyone so that non-interested users do not end up paying for a service they don't require.
	\item \label{goal: root} \textbf{Trust rooted in Hardware} In light of the many software based vulnerabilities discussed in Section \ref{docs:motivation}, the most viable option is to base the root of trust in hardware. This allows the user to rest assured that the trust is based in a temper resistant hardware module. It also decreases the trusted computing base (TCB) from hypervisors to a bare minimum. It further eliminates a large number of entities the user has to trust.
	\item \label{goal: chain} \textbf{Chain of Trust} Based on the previous design goal, the users should also be able to have a chain of trust in all the components taking part in the boot process. Starting from the hardware based root of trust, every subsequent component, from bootloaders to operating systems have to be measured or verified to build a chain of trust. This ensures that the boot sequence was not compromised on any stage.
	\item \label{goal: attest} \textbf{Attestation} A user should be able to have confidence in the root and chain of trust. This can only be achieved if the user can attest the different components involved in the chain himself without having to trust another entity to do it for him, such as the provider. 
	\item \label{goal: flex} \textbf{Flexibility} Different cloud users have different requirements and some like to use their own tools for provisioning or other tasks. Our service should not impose any limitations of what can be used and what cannot. Instead of building an enormous system which does everything from loading firmwares to installing operating systems, the service should be extremely light weight, only achieving the design goals and leaving everything else to the user. This would allow the clouds to house a diverse set of users.
	\item \label{goal: perf} \textbf{Performance} The service should not present a trade-off between performance and security for the user. The service should be able to accommodate interested users without imposing a high performance overhead.
\end{enumerate}

Based on the above discussed design goals, we built an architecture discussed in Section \ref{docs:arch}.

==> docs/impl_short.tex <==
\section{Implementation}\label{impl_sec}
By design, the architecture of Bolted is extremely flexible such that a tenant can choose the its trust level.
Bolted's flexibility also allows a tenant to pick and choose; the tenant is free to deploy all, some or none of the required components itself. There is also no restriction on how a component may be implemented as long as it provides the desired functionalty. This gives rise to a spectrum of possibilities ranging from full trust in provider to almost none. This allows different tenants with diverse trust requirements to use Bolted.


We have developed an open source implementation of each of these components. In particular: 
\textit{NERF} \cite{heads} provides a secure, small and reproducible firmware for the nodes.
\textit{Keylime} \cite{keylime} provides a distributed client-server attestation service. 
\textit{Hardware Isolation Service (HIL)} \cite{hil} is our implementation of the isolation service.
\textit{Bare Metal Imaging (BMI)} \cite{bmi} provides a fast provisioning service for bare metal node. Finally,
\textit{Bolted} implements an engine to orchestrate these services.
\textcolor{red}{Amin: provide url footnotes for each of these components.}

Figure \ref{fig:impl} shows all these services and their implementation details.
Each of these are described after discussion of the NERF firmware that we have developed and provides additional security. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{impl2.pdf} 
    \caption{Proposed Bolted implementation services and their details}
    \label{fig:impl}
\end{figure}

\subsection{NERF: the firmware}

Tenants who want secure attested nodes might be divided into three categories.
\begin{enumerate}
	\item Those who do not have access to firmware measurements.
	\item Those who do have access to firmware measurements but do not have access to firmware code so dont know what those measurements mean.
	\item Those who have access to the code and can calculate measurements on their own.
\end{enumerate}

Tenants who fall into the first category need to trust the provider for correct measurements. These measurements are then used to attest firmware, but the tenant has no way of determining the correctness of these measurements.

Tenants who fall in to the second category do not need to trust the cloud provider. They can provide their own measurements to the Attestation Service in order to ensure that the firmware is not compromised. Such tenants might have to trust a third party who provided those measurements though, such as the vendor who manufactured the node and flashed the firmware in to it in the first place.

Last category of tenants do not need to trust anyone. Since they have the code, they can deterministically build the firmware with the correct configurations and then measure it to produce the hashes. These values can then be used for attestation.

The NERF project aims to build an open, customizable, and slightly more secure firmware for server machines based on using Linux and Heads in the ROM to replace UEFI and Legacy BIOS as the bootloader. The most cautious tenants can use NERF as the firmware on their nodes.
%Unlike coreboot, NERF doesn't attempt to replace the chipset initialization code with opensource. 
%Instead it retains the vendor PEI (Pre-EFI environment) code as well as the signed ACM (authenticated code modules) that Intel provides for establishing the TXT (trusted execution environment). 
The NERF firmware replaces the DXE (Driver Execution Environment) portion of UEFI with a few open source wrappers, the Linux Kernel and the Heads measured runtime.

NERF has many advantages over the vendor UEFI firmware:
\begin{enumerate}
\item NERF is more secure. The Linux devices drivers and filesystems have had significantly more scrutiny than the UEFI implementations.
\item Its reproducible build allows remote attestation or TPM sealing.
\item It is open source and therefore, users can apply patches and build their own versions as well, instead of waiting for vendor update cycles.
\item It is significantly more flexible: it can use any Linux supported filesystem or device driver, execute Linux shell scripts to perform remote attestation over secure network protocols, mount encrypted drives, etc. This flexibility allows the firmware to easily be incorporated into a cloud provisioning system.
\item It is significantly faster to startup: the NERF interactive bash shell is ready in about 30 seconds after power on, compared to around 8 minutes for UEFI to boot into grub to load Linux.
\item NERF has a significantly smaller amount of untrusted binary blobs. Only a few hundred KB of closed-source code remain, compared to the 32 MB of UEFI binaries.

\end{enumerate}

We burnt NERF firmware into our Dell R630 server's Flash ROM. 
By reading originial firmware from the server, we were able to extract the required sections of the firmware and include it into NERF firmware. 
This requires physical access to the server. 

To make it usable for the tenants who don't have physical access to the servers, we have also booted NERF through netwrok boot (using iPXE protocol). 
This way, we do not need physical access to the server, however it increases the boot time significsntly since server should first boot up using its original firmware and then boot up using NERF.

\subsection{Keylime: attestation service}

In our implementation of Bolted, we used measured validation for attesting nodes. 
%As we discussed in section \ref{doc:background}, in measured method, the hash of the software component will be calculated and sent to a third party to be verified.
We have Keylime for this purpose. In this section, we first describe the architecture of Keylime and then how we adapted it for Bolted.

\subsubsection{Keylime architecture and implementation}

Keylime is a cloud key management system for secure provisioning and monitoring.
It leverages TPM technology \cite{tpm} to validate the integrity of software running on a cloud node.

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\linewidth]{Keylime.pdf} 
%    \caption{Keylime architecture}
%    \label{fig:keylime}
%    \includegraphics[width=\linewidth]{Keylime_2.pdf}
%\end{figure}

The key insight of Keylime is to utilize trusted computing to bootstrap identity in the cloud and provide integrity measurement to support revocation, but then allow high-level services that leverage these identities to operate independently. 

Keylime consists of three major components; Registrar, (b) Cloud Verifier and (c) Cloud Node.

The registrar stores and certifies the public \textit{AIKs} of the TPMs indexed by node UUID in the tenant's infrastructure. The tenant registrar can be hosted outside the cloud in the tenant's own infrastructure or could be hosted on a physical system in the cloud. The registrar is only a trust root and does not store any tenant secrets. Tenants request public \textit{AIKs} from the registrar through a server-authenticated TLS channel. The \textit{AIKs} in the registrar are validated through a TPM-compatible enrollment protocol.

The core component of keylime is an out of band Cloud Verifier (CV). As depicted in figure \ref{fig:impl}, each cloud organization will have at least one CV that is responsible for verifying the system state of the cloud node. The tenant can host the CV in the IaaS cloud or on premises at their own site. The CV relies upon the tenant registrar for validating that the \textit{AIKs} used to sign TPM quotes are valid.

The Keylime protocol uses secret sharing to rely upon the CV for integrity measurement. The protocol then extends beyond bootstrapping to enable continuous system integrity monitoring. The CV periodically polls each cloud node's integrity state to determine if any runtime policies have been violated. 


\subsubsection{Keylime for Bolted}

We create a chain of trust rooted in hardware. 
Using Keylime, we ensure that this chain is not broken in any stage.
%For doing this, Keylime incorporates TPM's PCR measurements for the coreboot, Heads, and Keylime. 
%Upon successful attestation, Keylime will bootstrap the tenant OS and measure it into a PCR allowing the tenant to perform future integrity tests.
After provisioning firmware (NERF) and Keylime client, Keylime checks the integrity of node's firmware and uploaded image including the client side of itself. If the node passed the attestation test, the tenant can attach it to its secure enclave. when OS is provisioned by provision service, Keylime first checks its integrity and if it is okay, OS image will be installed on the node.
It is also possible for tenant to measure the applications running on the OS and check their integrity.
Using the implemented attestation service, Tenant runs a safe application over a secure hardware which she knows that it is not compromised.

For doing these, a lightweight Keylime node configuration has been created that allows for Keylime to be loaded early in the boot process, such as in NERF, where important libraries like libc are not available in the system. This is a fully self-contained package made with the help of pyinstaller which allows the Keylime node software to be installed on a system without requiring additional dependencies. In this way, NERF can run the Keylime node software on bare metal, which will then obtain a decryption key and further provisioning from the Keylime verifier and tenant.


\subsection{HIL: the isolation service}

The Hardware Isolation Layer (HIL) architecture is first described before we show how it is used in the bolted implementation.

\subsubsection{HIL architecture and implementation}

HIL is designed to manage server resources in a multi-tenant data center, providing a fundamental allocation and isolation layer that allows reconfiguration of physical resources without manual administrative effort. 
%HIL takes a minimalist, ``exokernel"-like approach which helps users to trust to only a small amount of code to be trusted to provide the basic services.

%A large data center may contain multiple server pools, clusters, and compute services managed by different companies, institutions, or research groups.
%Each of these environments exists in a separate ``silo" of physical infrastructure.
%HIL can be used in such an environment to break these siloes to allow infrastructure to be moved to wherever it is needed. 
%In such a data center there would be multiple HIL service instances, one per server pool or administrative entity.
%For example, in our current environment, in addition to the production HIL deployment at Northeastern we have additional (experimental) HIL deployments at MIT and BU.

%Services like the MOC or compute clusters shared by multiple institutions can span these HIL instances, as shown in Figure \ref{fig:hil}. 

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\linewidth]{hil.pdf} 
%    \caption{HIL provides strong network-based isolation between flexibly-allocated pools of hardware resources, enabling normally incompatible provisioning engines (e.g. Ironic, MaaS, xCAT) to manage nodes in a data center.}
%    \label{fig:hil}
%\end{figure}

HIL needs little or no changes to the exsiting provisioning services (e.g., BMI, Ironic, xCAT and etc.) which interact directly with the allocated hardware.

The basic container for resources in HIL is the project, which have a set of users. 
Projects contain nodes and networks: nodes represent compute nodes, and are atomically allocated by assignment to a project; each node has a set of NICs which may be connected to networks.
Networks can either be private to a single project - e.g. used for the purpose of isolating communications - or public and accessible by all projects, as in the case of external internet access.

\if 0
The core components of HIL are those which are used in all projects (see Figure \ref{fig:impl}) .
There are three components: (a) the HIL server itself, implementing the HIL API, (b) the database, which persists HIL state and configuration, and (c) the operation engine, which sequences potentially long-running network operations.

\noindent\textbf{HIL Server:} this implements most of the HIL logic and exposes HIL's REST API, interfacing with the database, the operation engine, and the out-of-band management (OBM) drivers.

\noindent\textbf{OBM and Auth drivers:} The HIL server controls individual bare-metal nodes via the OBM driver, which provides functions to power cycle a node, force network booting, and access the serial console log.

\noindent\textbf{Operation Engine:} This is responsible for sequencing and coordinating operations which change network configuration. It receives requests from the API server via a queue, performs them in the order they were submitted and finally updates the database upon completion.

\noindent\textbf{Switch drivers:} These are used by the operation engine to implement the functions which manipulate network connectivity, with implementation (but not interface) varying by the network technology being used (e.g. VLAN), as well as vendor and model of the device being controlled. By manipulating network connectivity HIL is able to protect nodes within a project (or their management interfaces) against access from other projects or external systems.

\fi

\subsubsection{HIL for Bolted}

The network protection requirement can be implemented in two different ways. A tenant can use network isolation to be sure that its nodes and data are protected from other tenants. Whole enclave network will be isolated from other networks. The data inside the network will be secure. i

The Other way is to use network encryption (e.g., IPSec). All packets generated by the nodes will be encrypted by the keys known to the tenant and its trusted parties. 

A most cautious tenant can use network isolation with network encryption for more security. This way, any data between the nodes inside trsuted network will also be encrypted.

In Bolted we have used network isolation to isolates nodes and networks. 
Since this isolation layer is interacting with the providers physical switches, it has to be trusted and deployed by the provider. 
For reducing security risks, an isolation layer which has a very small trusted computing base (TCB) is more favorable. 
This is one of the reasons we chose HIL\cite{hil}. 
We previosly implemented HIL to enable agility in our datacenter. 
And in Bolted, we rely on HIL to provide network and node isolation during key stages. 
%As the source of truth for information on nodes,
%First, it ties each node's HIL identity to a TPM identity by exporting the TPM's public Endorsement Key (EK) through administrator-modifiable metadata per node, so that a tenant can have assurance that the node it is communicating with is the node it reserved. 
%Without this ability, the tenant would not know that the TPM it was in communication with belonged to the reserved node or a an attacker-controlled node. 
%HIL exposes the whitelist of TPM PCR measurements that relate to the platform components like BIOS/UEFI firmware and the firmware settings. 
%In this way, a tenant has knowledge of what the measurements should be by trusting the provider. 
%An alternative, where the list of good measurements were extracted from the node itself after it was acquired, could be viable on server platforms that offered sufficient firmware integrity mechanisms like reliable firmware overwriting.

%In order to support the needs of Bolted, HIL was modified to store provider-maintained, tenant-accessible key/value pairs for nodes to communicate expected firmware whitelist values so that tenants may verify the values in TPM attestations.


%For isolation service we chose HIL which guarantees to isolate different users' nodes from each other. 
%With a structure similar to Exokernel \ref{exokernel}, HIL isolates users enabling even small users that are security sensitive to carve their own secure enclave.

%In addition, HIL makes it possible to allocate bare-metal physical nodes while tenants can choose their own cloud orchestration and virtual layer. 
%HIL also supports users to choose their own provisioning systems, including BMI \ref{bmi}, Ironic \ref{ironic}, and Foreman \ref{foreman}.

%By choosing their own image, users can have their orchestration service to be deployed on top of their provisioned image. 
%This flexibility has another advantage. HIL brings simplicity to the provider's orchestration stack by only performing hardware isolation and leaving the rest under the tenant's control, supplying a minimal Trusted Computing Base for isolation between tenants.


\subsection{BMI: provisioning service}

In this section we first explain our provisioning service' structure and then describe the modifications we have done to BMI to use it in Bolted.

\subsubsection{BMI architecture and implementation}

For our infrastructure at MOC, we have implemented BMI to quickly provision bare metal nodes using diskless provisioning mechanisms.
Doing this, BMI stores images (user or BMI provided) in an image repository. When a provisioning API call is made for a bare-metal node with a given image, a linked-clone of that image is created, followed by network isolation of the requested bare-metal node and mounting of the clone on the bare-metal node. When the node network-boots, it only fetches the parts of the image it uses (less than 1\% of image is typically used), which significantly reduces the provisioning time.
This method is efficient such that BMI can provision tens of nodes under five minutes, and can decommission and re-purpose unused/underutilized nodes under 10 minutes. 
Moreover, with today's networks, and distributed file systems, accessing data over a network can be more efficient, avoids any single points of failures, and allows the tenant to recover from node failres \cite{ceph, MSFT_PAPER}.  %Cite here ceph paper and paper from MSFT research on file system for flat datacewnter.

%As shown in figure \ref{fig:impl} BMI has three major components: (a) Storage Service (CEPH), (b) iSCSI Service (TGT Server) and (c) Diskless Provisioning Service (PXE Server). 
%Similar to HIL, BMI follows a driver based approach, provides and isolates each component. 
%This allows BMI to be modified to support different storage services, or new iSCSI services to be adopted. 

\if 0
\noindent\textbf{Storage Service:} provides a data store for the cloud images and exposes API's to rapidly clone and snapshot existing images. In our implementation we use CEPH \cite{ceph} as our storage solution.

\noindent\textbf{iSCSI and Diskless Provisioning Services:} Our implementation of disk-less provisioning is based on network booting bare-metal nodes uding Preboot eXecution Environment (PXE). 
Ceph Block Device (RBD) based cloud images are exposed as iSCSI targets. 
Despite PXE specifications to support network booting from various targets (HTTP, iSCSI, AOE, etc.), it is up to the NIC manufacturer to implement the support into the NIC firmware. To ensure that BMI can provision any bare-metal node irrespective of the NIC firmware capabilities of that node, BMI first chainloads into iPXE \cite{iPXE}, which eventually network boots the bare-metal nodes from the exposed iSCSI target.

\noindent\textbf{BMI API Server:} API Server is a python based RESTful web service that controls the flow between different components of BMI. Exposed APIs enable users to (de)provision nodes, clone provisioned nodes, create snapshots of provisioned nodes, (de)register users, perform various operations pertaining to images (upload, download, rename, share, list, etc.), list various resources, etc.

\fi

\subsubsection{BMI for Bolted}

After attestation service, i.e., Keylime, attestes the node, tenant moves the node to its secure enclave. 
Since in Bolted architecture, tenant's network is isolated, it can implement its own provisioning service to upload OS and other softwares securly on the node. We used BMI for this purpose. 

Alternatively, if a tenant want to use provider's BMI, then it needs to encrypt its images and put them in shared provider storage. Using attestation service, the tenant bootstraps a key to get the machine out of the airlock state and then it can decrypt its disk image.  
A most cautious tenant, for super defense in depth, can implement both methods on top of one another.

BMI network boots machines using remotely mounted disk images. This provides more security by the fact that the entire state of the system is remote, reducing the chance of leaving something behind by accident.
In addition, in some of the use cases of Bolted, e.g., for emergency response, we want 100s of nodes provisioned rapidly.
BMI provides a good foundation for this, since it can provision nodes to previously used images in minutes, instead of standard provisioning tools (e.g., Ironic) that may take half hour or more. 
In addition, BMI entails much less bandwidth demands on the network than transferring many multi-gigabyte images over the network since it only fetches the required parts of the image.


%Three changes were made to BMI to function with Bolted. 1) A capability was added for BMI tenants to run scripts against a BMI-managed filesystem. This was needed in order to extract boot information (kernel, initramfs image and kernel command lines) from images so that they could be passed to a booting node in a secure way via Keylime. 2) Make HIL network assignment calls optional. 3) In cases where iPXE is used for BMI booting, an API was added to provide measurements so that they could be verified by Keylime.



\subsection{Bolted: Putting all together}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{boot_seq2.pdf} 
    \caption{Boot sequence for components. The authenticated code module (ACM) which executes and measures the boot block of NERF. This boot block measures the 2nd stage of NERF before launching it. NERF performs POST, executes the Head kernel and loads its initramfs after measuring them. Heads downloads the KeyLime client which is part of KeyLime Service that attests node on tenant's request. Once positive attestation acknowledgement is received, client sends the LUKS key along with script to download the client OS image. After measuring the script, it is executed which fetches the client OS image. Client OS image is measured and if it is found to be as expected, Heads launches into the Client OS environment}
    \label{fig:system}
\end{figure*}

For our implementation we targeted the boot sequence depicted in figure \ref{fig:system}. The Dell server boots into NERF's boot block from the legacy reset vector. This boot block measures itself before measuring and loading the NERF RAM stage. From that point on, each component is responsible for measuring the following component. Attestation using Keylime incorporates PCR measurements for the NERF and Keylime. Upon successful attestation Keylime will bootstrap the tenant OS and measure it into a PCR allowing the tenant to perform future integrity tests.


==> docs/motivation.tex <==
\section{Motivation}
\label{docs:motivation}

%Explain the problem and the need to have a secure cloud elastically. We need to talk about tenants such as AirForce and the possibility of using public cloud quickly in case of national disaster. 
\textcolor{blue}{Sahil: This being a short paper, I think introduction takes care of the motivation. We should remove this section from this paper.} \par
Benefits of using a public cloud are well known like on-demand elastic scaling, pay-as-you-go computing model, data redundancy, ease of collaboration, regular maintenance, upgrade of softwares and services offered by the cloud provider, etc. Despite of such obvious benefits many companies and government agencies still manage their critical applications and sensistive data privately.({cite the 4 reasons companies are reluctant to move}{cite getting cyber serious}). As reported in ({cite getting cyber serious}) the overall utilization of federal government managed data-centers is only 7\% while their power-consumption is upto 12 billion kilo watt hours of electricity per year. Large trusted computing base of virtualization based clouds combined with increased security risks due to multi-tenancy and lack of transparancy into the layers managed by the cloud provider are among the major barrier against moving critical applications from government and companies into the cloud. ({cite identifying risks associated with governmental use of cloud computing}{cite the DISA presentation}). Bolted helps in significantly reducing the security risks related to issues of multi-tenancy and trusted computing base while giving control akin to privately owned infrastructure. It can serve as a promising model to run mission critical services like first responder communication systems securely using public clouds ready to scale up rapidly in response to any national emergencies.

\textcolor{blue}{Sahil: Will work on the following points later}

Talk about the firmware (e.g., logacy BIOS and UEFI) vulnerability
Talk about open compute nodes and the possibilty of updating firmware on them. This feeature makes it possible to upload a secure firmware on the machine. 


==> docs/relatedWork.tex <==
\section{Related Work}\label{doc:relatedWork}

%Based on our paper story, we need to explain network management and configuration, storage encryption and network encryption related works. We also need to descrive related works in securing the cloud. 
Cloud computing inherits all the security risks of a traditional IT-infrastructure. 
With virtualization added to the trusted computing base along with introduction of multi-tenancy at the infrastructure layer has made public clouds further vulnerable to new types of attacks that were not previously possible in privately owned data-centers. 
  


%\subsection{Bare Metal and Virtualization}

%\subsection{Trust in cloud}

%\subsection{Security}

%\subsection{Secure Hardware}

%\subsection{Secure Isolated Enclaves in clouds}

%\subsection{Cloud Services}


==> outline <==
architecture:

Figure 1 - simple scenario

The architecgture of Bolted is shown in Figure X. There are four component micro-services:
1. The isolation service provides networks isolation between machines allocated to different users.
2. The attestation infrastructure~\cite{keylime},  leverages TPM technology to validate the integrity of all firmware and software running on a node, as well as providing a mechanism for secure communication of secrets for encryption of storage and communication.
3. The provisioing service installs a tenants software onto their nodes
4  The orchestration service that ties it together

- describe lifecycle first orchestration puts node into "airloc", a
  holding where they firmware can be validated before the node is
  allowed into the trused. In the airlock, initial software is loaded
  up that will send to the attestation service the signature of the
  firwmare..

Figure 2 - complex scenario

- describe the flexibility
The one component of the bolted architecture that needs to be deployed
by a provider is the isolation service, since it controls the physical
switches.


For implemennation

- first short overview our implementation of isolation service is
  HIL...The client side of attestation is deployed on a minimal linux
  we call HEADS

- section on each of HIL/Keylime/BMI/HEADS



